Quantum Theory Over Dual-Complex Numbers

We take quantum theory and replace C by C[e] where e^2 = 0, i.e. we extend quantum theory to the ring of dual complex numbers. The aim is to develop a common language in which to treat continuous quantum physics and discrete quantum models in a unified manner, including their symmetries. Since quantum theory is linear, introducing e is enough to model infinitesimals. A first objection to this programme is that C[e] is not a field, since division by e is undefined, while quantum mechanics typically relies on division. A second objection concerns whether unitarity still makes sense given e^2 = 0. Hence, the core of this work is dedicated to proving that dual-complex quantum theory remains fully consistent. In particular, norm is preserved at all times, and renormalization never requires dividing by an infinitesimal. An equivalence with conventional quantum theory is demonstrated: the dual-complex extension of a parametrized quantum operation automatically provides a linear treatment of its first-order variations. As a first example application, we provide a unified description of both the Dirac equation in the continuum and the Dirac Quantum Walk in the discrete. We establish the discrete Lorentz covariance of the latter.

==> eptcsdata.tex <==
\providecommand{\firstpage}{166}
\providecommand{\publicationstatus}{J. van de Wetering, O. Oreshkov, and A.B. Sainz (Eds.):\\
Quantum Physics and Logic 2026 (QPL 2026)\\
EPTCS 456, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.456.6}{10.4204/EPTCS.456.6}}
\pdfoutput=1

